Using Program Synthesis for Social Recommendations

This paper presents a new approach to select events of interest to a user in a social media setting where events are generated by the activities of the user's friends through their mobile devices. We argue that given the unique requirements of the social media setting, the problem is best viewed as an inductive learning problem, where the goal is to first generalize from the users' expressed "likes" and "dislikes" of specific events, then to produce a program that can be manipulated by the system and distributed to the collection devices to collect only data of interest. The key contribution of this paper is a new algorithm that combines existing machine learning techniques with new program synthesis technology to learn users' preferences. We show that when compared with the more standard approaches, our new algorithm provides up to order-of-magnitude reductions in model training time, and significantly higher prediction accuracies for our target application. The approach also improves on standard machine learning techniques in that it produces clear programs that can be manipulated to optimize data collection and filtering.

==> Makefile <==
PAPER=lifejoin
LATEX=`which pdflatex`
BIBTEX=`which bibtex`

#FIGURES=thttpdConstraints.pdf bbrOverview.pdf

FIGURES=figures/*.pdf

all: $(PAPER).pdf

$(PAPER).pdf: $(PAPER).tex $(PAPER).bib \
              abstract.tex intro.tex overview.tex macros.tex \
							plApproach.tex hybridApproach.tex times-lite.sty ttquot.sty \
              relatedWork.tex experiments.tex conclusions.tex $(FIGURES)
							$(LATEX) $<
							$(BIBTEX) $(PAPER)
							$(LATEX) $<
							$(LATEX) $<


clean:
	rm -f *.out *.bak *.dvi *.aux *.log *.blg *.bbl $(PAPER).pdf

spell:
	@ for i in *.tex; do aspell -t $(ASPELL_CMDS) -p ./aspell.words -c $$i; done
	@ ( head -1 aspell.words ; tail -n +2 aspell.words | sort ) > aspell.words~
	@ mv aspell.words~ aspell.words


